Compact Scene Graphs for Layout Composition and Patch Retrieval

Structured representations such as scene graphs serve as an efficient and compact representation that can be used for downstream rendering or retrieval tasks. However, existing efforts to generate realistic images from scene graphs perform poorly on scene composition for cluttered or complex scenes. We propose two contributions to improve the scene composition. First, we enhance the scene graph representation with heuristic-based relations, which add minimal storage overhead. Second, we use extreme points representation to supervise the learning of the scene composition network. These methods achieve significantly higher performance over existing work (69.0% vs 51.2% in relation score metric). We additionally demonstrate how scene graphs can be used to retrieve pose-constrained image patches that are semantically similar to the source query. Improving structured scene graph representations for rendering or retrieval is an important step towards realistic image generation.

==> tex/results/scene_layout_results.tex <==
\begin{figure*}[!t] \begin{center}
    \includegraphics[width=\textwidth]{images/layout_images/CEFRL_layout_prediction.png}
    \caption{Extreme point supervision and extreme point conditioned mask prediction yields improved layout prediction from scene graph. For each (a)input scene graph, predicted extreme points per objects using the proposed method is shown in (d). For better visualization, the octagonal mask around the extreme points for each \emph{object} category and the bounding box around the octagon masks for all \emph{object} and \emph{stuff} categories are shown. Column (e) shows the scene layout mask predicted by our model vs the (f) layout predicted by JJ~\cite{img_gen_from_scene_graph18}. For reference, the ground truth extreme points and their connecting octagons overlaid on the corresponding ground truth image are shown. Proposed model handles placements of multiple objects (row 1), inter-class spatial arrangement (row 2) and overall learns better shapes.   
}  
\label{fig:layout}
\end{center}
\end{figure*}

==> tex/results/visual_comparison_coco.tex <==
\newcommand{\vcs}{0.18}

\begin{figure*}[!t] \begin{center}
\begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000028_layout.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000028_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000028_gtbm.png}
  \end{subfigure}
\begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000028_gt_img.png}
  \end{subfigure}
  
  \begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000028_layout_jj.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000028_img_jj.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000028_gtbm_jj.png}
  \end{subfigure}
\begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000028_gt_img.png}
  \end{subfigure}
   \vspace{3.00mm}
      
      
\begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000734_layout.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000734_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000734_gtbm.png}
  \end{subfigure}
\begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000734_gt_img.png}
  \end{subfigure}
  
  \begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000734_layout_jj.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000734_img_jj.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000734_gtbm_jj.png}
  \end{subfigure}
\begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000734_gt_img.png}
  \end{subfigure}
  \vspace{3.00mm}

\begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000897_layout.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000897_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000897_gtbm.png}
  \end{subfigure}
\begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000897_gt_img.png}
  \end{subfigure}
  
  \begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000897_layout_jj.png}
        \caption{Predicted layout}
  \end{subfigure}
  \begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000897_img_jj.png}
    \caption{Generated Image}
  \end{subfigure}
  \begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000897_gtbm_jj.png}
    \caption{With GT layout}
  \end{subfigure}
\begin{subfigure}[b]{\vcs\textwidth}
    \includegraphics[width=\textwidth]{images/coco/000897_gt_img.png}
    \caption{Ground truth}
  \end{subfigure}
\caption{Examples from COCO-stuff. Sample results of layout prediction, image generation, image generation with ground truth layout for query scene graphs from COCO-stuff test set. For each pair of rows, the top corresponds to our model, and the bottom to results from Johnson \etal \cite{img_gen_from_scene_graph18}. In these anecdotal examples, scene context helps ensure better layout prediction and generation of more realistic images.}  
\label{fig:coco}
\end{center}\end{figure*}






